Lepton polarization asymmetries in rare semi-tauonic $ b \rightarrow s $ exclusive decays at FCC-$ee$

We consider measurements of exclusive rare semi-tauonic $b$-hadron decays, mediated by the $b \rightarrow s \tau^+ \tau^-$ transition, at a future high energy circular electron-positron collider (FCC-$ee$). We argue that the high boosts of $b$-hadrons originating from on-shell $Z$ boson decays allow for a full reconstruction of the decay kinematics in hadronic $\tau$ decay modes (up to discrete ambiguities). This, together with the potentially large statistics of $Z\to b\bar b$, opens the door for the experimental determination of $\tau$ polarizations in these rare $b$-hadron decays. In light of the current experimental situation on lepton flavor universality in rare semileptonic $B$ decays, we discuss the complementary short-distance physics information carried by the $\tau$ polarizations and suggest suitable theoretically clean observables in the form of single- and double-$\tau$ polarization asymmetries.

==> Section2/Section2bib.tex <==
%
% Citations for Section 2 
%
@article{Gomez-Ceballos:2013zzn,
      author         = "Bicer, M. and others",
      title          = "{First Look at the Physics Case of TLEP}",
      booktitle      = "{Proceedings, 2013 Community Summer Study on the Future
                        of U.S. Particle Physics: Snowmass on the Mississippi
                        (CSS2013): Minneapolis, MN, USA, July 29-August 6, 2013}",
      collaboration  = "TLEP Design Study Working Group",
      journal        = "JHEP",
      volume         = "01",
      year           = "2014",
      pages          = "164",
      doi            = "10.1007/JHEP01(2014)164",
      eprint         = "1308.6176",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      SLACcitation   = "%%CITATION = ARXIV:1308.6176;%%"
}


@article{Behnke:2013lya,
      author         = "Abramowicz, Halina and others",
      editor         = "Behnke, Ties and Brau, James E. and Burrows, Philip N.
                        and Fuster, Juan and Peskin, Michael and Stanitzki, Marcel
                        and Sugimoto, Yasuhiro and Yamada, Sakue and Yamamoto,
                        Hitoshi",
      title          = "{The International Linear Collider Technical Design
                        Report - Volume 4: Detectors}",
      year           = "2013",
      eprint         = "1306.6329",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      reportNumber   = "ILC-REPORT-2013-040, ANL-HEP-TR-13-20,
                        BNL-100603-2013-IR, IRFU-13-59, CERN-ATS-2013-037,
                        COCKCROFT-13-10, CLNS-13-2085, DESY-13-062,
                        FERMILAB-TM-2554, IHEP-AC-ILC-2013-001, INFN-13-04-LNF,
                        JAI-2013-001, JINR-E9-2013-35, JLAB-R-2013-01,
                        KEK-REPORT-2013-1, KNU-CHEP-ILC-2013-1, LLNL-TR-635539,
                        SLAC-R-1004, ILC-HIGRADE-REPORT-2013-003",
      SLACcitation   = "%%CITATION = ARXIV:1306.6329;%%"
}

